A generalization of Rasmussen's invariant, with applications to surfaces in some four-manifolds

We extend the definition of Khovanov-Lee homology to links in connected sums of $S^1 \times S^2$'s, and construct a Rasmussen-type invariant for null-homologous links in these manifolds. For certain links in $S^1 \times S^2$, we compute the invariant by reinterpreting it in terms of Hochschild homology. As applications, we prove inequalities relating the Rasmussen-type invariant to the genus of surfaces with boundary in the following four-manifolds: $B^2 \times S^2$, $S^1 \times B^3$, $\mathbb{CP}^2$, and various connected sums and boundary sums of these. We deduce that Rasmussen's invariant also gives genus bounds for surfaces inside homotopy 4-balls obtained from $B^4$ by Gluck twists. Therefore, it cannot be used to prove that such homotopy 4-balls are non-standard.

==> sections/sec-GenusBounds.tex <==
\section{OLD SECTION --- TO BE DISTRIBUTED AMONG OTHER SECTIONS} \label{sec:genus bounds}

In \cite{Rasmussen}, $s(K)$ is used to bound surfaces in $B^4$ bounded by knots $K$ in $S^3$.  The argument is generalized to involve oriented cobordisms between links in CITE BW.  The main ingredient in those proofs involves ensuring that certain oriented cobordisms between oriented links send Lee generators to (non-zero multiples of) Lee generators.  If we wish to mimic those ideas for a link in $M^r=\#^r(S^1\times S^2)$ bounding a surface in some 4-manifold $W$ with boundary $M^r$, we will need to understand some more details on where Lee generators appear in the complex $\LC{\infFT}$ and how they are affected by oriented cobordisms.

\subsection{Oriented cobordisms}

\subsection{Genus bounds in $M^r \times I$}

We get a bound
$$ |s(L)| \leq g_{S^1 \times S^2 \times I}$$

This is the same as for surfaces in $S^1 \times B^3$. We could get a (potentially) better bound by defining
$$ s^+(L) = -s(m(L))$$
where $m(L)$ is the mirror of $L$. Applying the inequality above to $m(L)$ we get it with $s^+$ instead of $s^-$. 

When $L$ is a knot, we have $s=s^+$. For links with two components, $s$ and $s^+$ are the analogues of $\tau^-$ and $\tau^+$ in knot Floer homology. In knot Floer homology, $\tau^{\pm}$ of a link is the same as that of its knotification, but for $s$ and $s^+$ they are different. (Compare the unknot and Hopf link.)

For links of two components, since there are annuli between $L \sqcup m(L)$ and $\emptyset$, we have
$$ s_+(L) \geq s_-(L) - 2.$$
We may hope to prove $s_+(L) \geq s_-(L)$.

\subsection{The general principle}
Suppose we have a four-manifold $W$ with boundary $M^r$, such that $W$ is constructed with no three-handles. (Thus, we could construct a closed four-manifold from $W$ by adding three-handles and a four-handle.) 

Suppose we have a link $L \subset \del W$ and a properly, smoothly embedded surface $\Sigma \subset W$ with $\del \Sigma = L$. To get a bound on the genus of $\Sigma$, we can intersect it with a neighborhood of the $2$-skeleton of $W$. We get a cobordism from $L$ to a cable of the link in $M^s$ given by the attaching spheres of the $2$-handles. Thus, we are interested in computing the $s$-invariants of those cables.

This is related to what was attempted in \cite{mnm}.

\subsection{Genus bounds in $D^2 \times S^2$}

$$\frac{s}{2} \leq g_{S^2 \times D^2} \leq g_{S^1 \times B^3}.$$

\subsection{Genus bounds in $\CP$}

\subsection{Genus bounds in connected sums}

\begin{corollary}
Suppose $X$ is a homotopy $4$-ball such that $X \# \bCP =B^4 \# \bCP$. Let $K \subset \del X = S^3$ be a knot that bounds a smoothly, properly embedded surface $\Sigma \subset X$ of genus $g$. Then
$$ s(K) \leq 2g.$$
\end{corollary}

\begin{corollary}
Suppose $X$ is a homotopy $4$-ball such that $X \# \bCP =B^4 \# \bCP$ and $X \# \CP =B^4 \# \CP$. (For example, this is true if $X$ is obtained from $B^4$ by a Gluck twist.) Let $K \subset \del X = S^3$ be a knot that bounds a smoothly, properly embedded disk $D \subset X$. Then $s(K)=0$.
\end{corollary}

This shows that the strategy for disproving the smooth four-dimensional Poincare conjecture that was outlined in \cite{mnm} cannot work for homotopy $4$-spheres that are obtained from $S^4$ by Gluck twists.

The same corollaries work for links that are weakly slice, i.e. bound a planar embedded surface. Apply the $s$-inequality to both $L$ and $m(L)$. We get
$$ s(L) \leq 1-\ell, \ \ s(m(L)) \leq 1-\ell,$$
but we know
$$ s(L) + s(m(L)) \geq 2-2\ell$$
from considering $\ell$ pairs of pants joining $L \sqcup m(L)$ to the unlink of $\ell$ components. This shows
$$ s(L)=1-\ell.$$

\subsection{The slice-Bennequin inequality in $S^1 \times S^2$} If we can give a combinatorial proof, that would be great.

